Variability Abstraction and Refinement for Game-based Lifted Model Checking of full CTL (Extended Version)

Variability models allow effective building of many custom model variants for various configurations. Lifted model checking for a variability model is capable of verifying all its variants simultaneously in a single run by exploiting the similarities between the variants. The computational cost of lifted model checking still greatly depends on the number of variants (the size of configuration space), which is often huge. One of the most promising approaches to fighting the configuration space explosion problem in lifted model checking are variability abstractions. In this work, we define a novel game-based approach for variability-specific abstraction and refinement for lifted model checking of the full CTL, interpreted over 3-valued semantics. We propose a direct algorithm for solving a 3-valued (abstract) lifted model checking game. In case the result of model checking an abstract variability model is indefinite, we suggest a new notion of refinement, which eliminates indefinite results. This provides an iterative incremental variability-specific abstraction and refinement framework, where refinement is applied only where indefinite results exist and definite results from previous iterations are reused.

==> conclusion.tex <==

In this work we present a game-based lifted model checking for abstract variability models with
respect to the full CTL. We also suggest
an automatic refinement procedure, in case the model checking result is indefinite.
We use the indefinite part of the colored game-graph of an abstract model to derive a failure node
and a reason, which are then exploited for refinement. 

The focus here is on verifying CTL properties in order to demonstrate this approach. Still,
the defined abstract variability models preserve the full $\mu$-calculus as well \cite{fase18}.
Since the game-based model checking \cite{DBLP:journals/iandc/ShohamG10,DBLP:series/txcs/Stirling01} is defined for $\mu$-calculus properties, we can easily adapt our approach for their verification as well.

The work \cite{DBLP:conf/tacas/ShohamG04} generalizes the definition of abstract models 
over 3-valued semantics by using the notion of hypertransitions. 
This results in more precise abstract models in which more CTL properties 
can be proved or disproved. In future, we can pursue this line of work by defining 
hypertransitions for our abstract variability models in order to obtain more precise results. 
